A Survey of Foundation Model-Powered Recommender Systems: From Feature-Based, Generative to Agentic Paradigms

Recommender systems (RS) have become essential in filtering information and personalizing content for users. RS techniques have traditionally relied on modeling interactions between users and items as well as the features of content using models specific to each task. The emergence of foundation models (FMs), large scale models trained on vast amounts of data such as GPT, LLaMA and CLIP, is reshaping the recommendation paradigm. This survey provides a comprehensive overview of the Foundation Models for Recommender Systems (FM4RecSys), covering their integration in three paradigms: (1) Feature-Based augmentation of representations, (2) Generative recommendation approaches, and (3) Agentic interactive systems. We first review the data foundations of RS, from traditional explicit or implicit feedback to multimodal content sources. We then introduce FMs and their capabilities for representation learning, natural language understanding, and multi-modal reasoning in RS contexts. The core of the survey discusses how FMs enhance RS under different paradigms. Afterward, we examine FM applications in various recommendation tasks. Through an analysis of recent research, we highlight key opportunities that have been realized as well as challenges encountered. Finally, we outline open research directions and technical challenges for next-generation FM4RecSys. This survey not only reviews the state-of-the-art methods but also provides a critical analysis of the trade-offs among the feature-based, the generative, and the agentic paradigms, outlining key open issues and future research directions.

==> Tables/dataset_table.tex <==

% \begin{table*}[htbp]
% \centering
% \caption{The list of most commonly used datasets in the Fashion RS literature.}
% \label{tab:datasets}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|c|c|c|c} 
% \hline
% \multicolumn{1}{c|}{\textbf{Dataset}} & \textbf{Reference} & \textbf{Availability} & \textbf{Size} & \multicolumn{1}{c}{\textbf{Area}} \\ 
% \hline
% ~Amazon Reviews & \href{http://jmcauley.ucsd.edu/data/amazon/links.html}{Link} & Yes & 140 million interactions & Generic \\ 
% \hline
% ~ DeepFashion~ ~ ~ & \cite{liu2016deepfashion} & No & 8 hundred thousand images & Generic \\ 
% \hline
% ~ ~Exact Street2Shop & \href{http://www.tamaraberg.com/street2shop/}{Link} & Yes & - & Street and shop photos \\ 
% \hline
% ~ ~ ~ExpFashion~ ~ ~ & \cite{DBLP:journals/tkde/LinRCRMR20} & No & 200k images and 1 million comments & Item \\ 
% \hline
% ~ ~Fashion IQ~ ~ ~ & \cite{DBLP:conf/cvpr/WuGGARGF21} & Yes & 77.6K images and textual descriptions & Dresses, shirts, tops\&tees \\ 
% \hline
% ~ ~FashionVC~ ~ ~ & \cite{10.1145/3123266.3123314} & No & 20~thousand images & Outfits by fashion experts \\ 
% \hline
% ~ ~ Fashion-136K~ ~ ~ & \cite{DBLP:journals/corr/JagadeeshPBDS14} & No & - & Fashion models \\ 
% \hline
% IQON3000 & \cite{DBLP:conf/mm/SongHLCXN19} & Yes & 300K outfits, by 3.5K users & Outfits \\ 
% \hline
% Polyvore & \cite{DBLP:conf/mm/HuYD15} & No & - & Item photos \\ 
% \hline
% Pog & \href{https://github.com/wenyuer/POG}{Link} & Yes & 4 millions images and descriptions & Item and Outfit \\ 
% \hline
% ~ ~ StyleReference~ ~ ~ & \cite{DBLP:journals/tmm/HidayatiGCHSWHT21} & No & 2~thousand pictures & Body features \\ 
% \hline
% ~ ~ ~ ~Style4BodyShape~ ~ ~ & \cite{DBLP:conf/mm/HidayatiHCHFC18} & No & 3150 celebrity records & Female celebrities \\
% \hline
% \end{tabular}
% }
% \end{table*}


\begin{table*}[t!]
\centering
\begin{tabular}{cccccc}
\toprule
\textbf{Dataset} & \textbf{Reference} & \textbf{Availability} & \textbf{Size} & \textbf{Area} \\
\midrule
Amazon Reviews & \href{http://jmcauley.ucsd.edu/data/amazon/links.html}{Link} & Yes & 140 million interactions & E-commerce \\
MovieLens & \href{https://movielens.org/}{Link} & Yes & - & Movie \\
BookCrossing & \href{https://www.bookcrossing.com/}{Link} & Yes & - & Book \\
Tenrec & \href{https://static.qblv.qq.com/qblv/h5/algo-frontend/tenrec_dataset.html}{Link} & Yes & - & Video \\


\bottomrule
\end{tabular}
\vspace{0.5cm} % Adjust the value as needed
\caption{The list of most commonly used datasets in the FM4RecSys literature.}
\label{tab:datasets}
\end{table*}



==> Tables/traditional_data.tex <==
% \begin{table*}[ht]
% \centering
% \begin{tabular}{|l|l|l|}
% \toprule
% \midrule
% \textbf{Data Sources/Tasks} & \textbf{Notes} & \textbf{Publications} \\ \hline
% Sequential Information & w/t User ID & \{16, 29, 33, 35, 73, 91, 117, 133, 143, 160, 173, 175, 189, 194, 198, 205\} \\ \cline{2-3} 
%  & Session-based w/o User ID & \{55--57, 68, 73, 99, 101, 102, 117, 142, 148, 149\} \\ \cline{2-3} 
%  & Check-In, POI & \{150, 151, 165, 185\} \\ \hline
% Text & Hash Tags & \{44, 110, 118, 158, 182, 183, 193, 209\} \\ \cline{2-3} 
%  & News & \{10, 12, 113, 135, 169, 200\} \\ \cline{2-3} 
%  & Review texts & \{11, 87, 126, 146, 174, 197, 202\} \\ \cline{2-3} 
%  & Quotes & \{82, 141\} \\ \hline
% Images & Visual features & \{2, 14, 25, 49, 50, 84, 98, 105, 112, 165, 172, 179, 191, 192, 197, 206\} \\ \hline
% Audio & Music & \{95, 153, 167, 168\} \\ \hline
% Video & Videos & \{14, 17, 27, 83\} \\ \hline
% Networks & Citation Network & \{9, 38, 66\} \\ \cline{2-3} 
%  & Social Network & \{32, 116, 166\} \\ \hline
% Cross Domain &  & \{39, 92, 166\} \\ \hline
% Others & Cold-start & \{154, 156, 170, 171\} \\ \cline{2-3} 
%  & Multitask & \{5, 73, 87, 174, 187\} \\ \cline{2-3} 
%  & Explainability & \{87, 126\} \\ \hline
% \end{tabular}
% \caption{Data Sources and Related Publications}
% \label{tab:data_sources}
% \end{table*}
\begin{table*}[ht]
\centering
\begin{tabular}{lll}
\toprule
\textbf{Data Sources/Tasks} & \textbf{Notes} & \textbf{Representative Publications} \\ 
\midrule
\midrule
Sequential Information & w/t User ID & \{16, 29, 33, 35, 73, 91, 117, 133, 143, 160, 173, 175, 189, 194, 198, 205\} \\ 
% \cmidrule(l){2-3} 
 & Session-based w/o User ID & \{55--57, 68, 73, 99, 101, 102, 117, 142, 148, 149\} \\ 
% \cmidrule(l){2-3} 
 & Check-In, POI & \{150, 151, 165, 185\} \\ 
\midrule
Text & Hash Tags & \{44, 110, 118, 158, 182, 183, 193, 209\} \\ 
% \cmidrule(l){2-3} 
 & News & \{10, 12, 113, 135, 169, 200\} \\ 
% \cmidrule(l){2-3} 
 & Review texts & \{11, 87, 126, 146, 174, 197, 202\} \\ 
% \cmidrule(l){2-3} 
 & Quotes & \{82, 141\} \\ 
\midrule
Images & Visual features & \{2, 14, 25, 49, 50, 84, 98, 105, 112, 165, 172, 179, 191, 192, 197, 206\} \\ 
\midrule
Audio & Music & \{95, 153, 167, 168\} \\ 
\midrule
Video & Videos & \{14, 17, 27, 83\} \\ 
\midrule
Networks & Citation Network & \{9, 38, 66\} \\ 
% \cmidrule(l){2-3} 
 & Social Network & \{32, 116, 166\} \\ 
% \cmidrule(l){2-3} 
 & Cross Domain & \{39, 92, 166\} \\ 
\midrule
Others & Cold-start & \{154, 156, 170, 171\} \\ 
% \cmidrule(l){2-3} 
 & Multitask & \{5, 73, 87, 174, 187\} \\ 
% \cmidrule(l){2-3} 
 & Explainability & \{87, 126\} \\ 
\bottomrule
\end{tabular}
\vspace{1em}
\caption{Data Sources and Related Publications}
\label{tab:data_sources}
\end{table*}

